Kullback-Leibler Divergence-Based Out-of-Distribution Detection with Flow-Based Generative Models

Recent research has revealed that deep generative models including flow-based models and Variational Autoencoders may assign higher likelihoods to out-of-distribution (OOD) data than in-distribution (ID) data. However, we cannot sample OOD data from the model. This counterintuitive phenomenon has not been satisfactorily explained and brings obstacles to OOD detection with flow-based models. In this paper, we prove theorems to investigate the Kullback-Leibler divergence in flow-based model and give two explanations for the above phenomenon. Based on our theoretical analysis, we propose a new method \PADmethod\ to leverage KL divergence and local pixel dependence of representations to perform anomaly detection. Experimental results on prevalent benchmarks demonstrate the effectiveness and robustness of our method. For group anomaly detection, our method achieves 98.1\% AUROC on average with a small batch size of 5. On the contrary, the baseline typicality test-based method only achieves 64.6\% AUROC on average due to its failure on challenging problems. Our method also outperforms the state-of-the-art method by 9.1\% AUROC. For point-wise anomaly detection, our method achieves 90.7\% AUROC on average and outperforms the baseline by 5.2\% AUROC. Besides, our method has the least notable failures and is the most robust one.

==> results/S2/glow_celeba32_vs_cifar100_EER_bs_5_10_S2.tex <==
& \textbf{2.8$\pm$0.2} & 82.9$\pm$0.1 & \textbf{0.0$\pm$0.0} & 91.6$\pm$0.5 \\

==> results/S2/glow_celeba32_vs_cifar100_bs_2_10_S2.tex <==
& \textbf{94.7$\pm$0.3} & \textbf{95.4$\pm$0.3} & 23.3$\pm$0.3 & 35.4$\pm$0.1 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 2.0$\pm$0.1 & 30.8$\pm$0.0 \\

==> results/S2/glow_celeba32_vs_cifar10_EER_bs_5_10_S2.tex <==
& \textbf{3.2$\pm$0.3} & 85.1$\pm$0.6 & \textbf{0.1$\pm$0.1} & 93.1$\pm$0.6 \\

==> results/S2/glow_celeba32_vs_cifar10_bs_2_10_S2.tex <==
& \textbf{93.3$\pm$0.3} & \textbf{94.0$\pm$0.2} & 19.6$\pm$0.1 & 34.1$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 1.0$\pm$0.1 & 30.7$\pm$0.0 \\

==> results/S2/glow_celeba32_vs_constant_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_celeba32_vs_constant_category_I_bs_2_4_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_celeba32_vs_constant_category_I_bs_5_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_celeba32_vs_imagenet32_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 26.4$\pm$0.2 & \textbf{0.0$\pm$0.0} & 20.7$\pm$0.8 \\

==> results/S2/glow_celeba32_vs_imagenet32_bs_2_10_S2.tex <==
& \textbf{99.5$\pm$0.1} & \textbf{99.5$\pm$0.0} & 71.0$\pm$0.1 & 76.4$\pm$0.1 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 87.9$\pm$0.3 & 90.5$\pm$0.2 \\

==> results/S2/glow_celeba32_vs_imagenet32_gray_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 6.6$\pm$0.1 & \textbf{0.0$\pm$0.0} & 1.6$\pm$0.2 \\

==> results/S2/glow_celeba32_vs_imagenet32_gray_bs_2_10_S2.tex <==
& \textbf{98.7$\pm$0.1} & \textbf{98.9$\pm$0.1} & 39.7$\pm$0.2 & 45.6$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 22.5$\pm$0.3 & 36.0$\pm$0.2 \\

==> results/S2/glow_celeba32_vs_imagenet32_gray_bs_2_4_S2.tex <==
& \textbf{97.5$\pm$0.1} & \textbf{97.7$\pm$0.0} & 43.2$\pm$0.1 & 48.4$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 37.9$\pm$0.2 & 45.0$\pm$0.2 \\

==> results/S2/glow_celeba32_vs_imagenet32_gray_bs_5_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 35.8$\pm$0.3 & 43.5$\pm$0.4 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 30.2$\pm$0.2 & 40.1$\pm$0.5 \\

==> results/S2/glow_celeba32_vs_svhn_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 28.5$\pm$0.2 & \textbf{0.0$\pm$0.0} & 22.0$\pm$0.4 \\

==> results/S2/glow_celeba32_vs_svhn_bs_2_10_S2.tex <==
& \textbf{99.9$\pm$0.0} & \textbf{99.9$\pm$0.0} & 73.0$\pm$0.1 & 67.3$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 91.6$\pm$0.4 & 90.3$\pm$0.8 \\

==> results/S2/glow_celeba32_vs_svhn_divergence_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 90.0$\pm$0.4 & \textbf{0.0$\pm$0.0} & 97.0$\pm$0.3 

==> results/S2/glow_celeba32_vs_svhn_divergence_bs_2_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 17.7$\pm$0.2 & 33.6$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 1.5$\pm$0.1 & 30.8$\pm$0.0 \\

==> results/S2/glow_celeba32_vs_uniform_noise_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_celeba32_vs_uniform_noise_gray_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 71.0$\pm$0.5 & \textbf{0.0$\pm$0.0} & 78.3$\pm$0.6 \\

==> results/S2/glow_cifar10_vs_CIFAR100_bs_2_10_S2.tex <==
& 54.6$\pm$0.0 & 54.9$\pm$0.2 & 53.7$\pm$0.0 & 54.4$\pm$0.0 & 57.2$\pm$0.6 & 56.8$\pm$0.5 & 56.1$\pm$0.0 & 57.0$\pm$0.0 \\

==> results/S2/glow_cifar10_vs_CIFAR100_bs_2_4_S2.tex <==
& \textbf{54.8$\pm$0.3} & \textbf{55.0$\pm$0.4} & 54.0$\pm$0.2 & 54.8$\pm$0.3 & \textbf{54.8$\pm$0.5} & 55.1$\pm$0.5 & 54.6$\pm$0.4 & \textbf{55.6$\pm$0.2} \\

==> results/S2/glow_cifar10_vs_CIFAR100_bs_5_10_S2.tex <==
& \textbf{55.4$\pm$0.2} & 55.8$\pm$0.5 & 54.6$\pm$0.8 & \textbf{55.9$\pm$0.5} & \textbf{57.0$\pm$0.9} & \textbf{57.9$\pm$1.0} & 55.7$\pm$0.3 & 56.9$\pm$0.4 \\

==> results/S2/glow_cifar10_vs_CelebA32_EER_bs_5_10_S2.tex <==
& 3.9$\pm$0.2 & \textbf{0.9$\pm$0.1} & 0.4$\pm$0.1 & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_cifar10_vs_CelebA32_bs_2_10_S2.tex <==
& 93.2$\pm$0.1 & 94.4$\pm$0.1 & \textbf{98.1$\pm$0.0} & \textbf{98.1$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_cifar10_vs_CelebA32_grey_EER_bs_5_10_S2.tex <==
& \textbf{23.3$\pm$0.7} & 65.5$\pm$0.6 & \textbf{13.4$\pm$0.5} & 69.5$\pm$0.8 \\

==> results/S2/glow_cifar10_vs_Constant_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_cifar10_vs_Imagenet32_EER_bs_5_10_S2.tex <==
& 18.9$\pm$0.6 & \textbf{3.8$\pm$0.3} & 12.3$\pm$0.6 & \textbf{0.8$\pm$0.1} \\

==> results/S2/glow_cifar10_vs_Imagenet32_bs_2_10_S2.tex <==
& 82.9$\pm$0.1 & 85.8$\pm$0.1 & \textbf{93.3$\pm$0.0} & \textbf{94.8$\pm$0.0} & 94.8$\pm$0.2 & 96.0$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_cifar10_vs_Imagenet32_grey_EER_bs_5_10_S2.tex <==
& \textbf{35.3$\pm$0.6} & 57.1$\pm$0.5 & \textbf{32.6$\pm$1.3} & 64.0$\pm$0.7 \\

==> results/S2/glow_cifar10_vs_SVHN_EER_bs_5_10_S2.tex <==
& 8.0$\pm$0.2 & \textbf{5.6$\pm$0.2} & 2.5$\pm$0.4 & \textbf{1.1$\pm$0.2} \\

==> results/S2/glow_cifar10_vs_SVHN_bs_2_10_S2.tex <==
& 89.8$\pm$0.1 & \textbf{90.6$\pm$0.1} & \textbf{91.2$\pm$0.0} & 87.6$\pm$0.0 & 99.8$\pm$0.1 & 99.8$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_cifar10_vs_SVHN_divergence_EER_bs_5_10_S2.tex <==
& \textbf{0.2$\pm$0.1} & 61.3$\pm$0.4 & \textbf{0.0$\pm$0.0} & 67.0$\pm$0.6 

==> results/S2/glow_cifar10_vs_Uniform_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_cifar10_vs_Uniform_gray_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 85.9$\pm$0.5 & \textbf{0.0$\pm$0.0} & 87.5$\pm$1.0 \\

==> results/S2/glow_cifar10_vs_tinyimagenet_bs_2_4_S2.tex <==
& \textbf{92.6$\pm$0.2} & \textbf{93.1$\pm$0.2} & 79.5$\pm$0.2 & 80.7$\pm$0.2 & \textbf{98.2$\pm$0.2} & \textbf{98.3$\pm$0.2} & 89.3$\pm$0.2 & 89.9$\pm$0.2 \\

==> results/S2/glow_cifar10_vs_tinyimagenet_bs_5_10_S2.tex <==
& \textbf{99.1$\pm$0.1} & \textbf{99.2$\pm$0.1} & 92.1$\pm$0.3 & 92.5$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 97.8$\pm$0.2 & 97.8$\pm$0.2 \\

==> results/S2/glow_cifar10_vs_uniform_gray_bs_2_4_S2.texglow_cifar10_vs_Constant_bs_2_4_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 9.9$\pm$0.0 & 32.5$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 11.2$\pm$0.0 & 32.8$\pm$0.0 \\

==> results/S2/glow_fashionmnist_vs_constant_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 54.2$\pm$0.4 & \textbf{0.0$\pm$0.0} & 53.9$\pm$0.8 \\

==> results/S2/glow_fashionmnist_vs_constant_category_I_bs_2_4_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 64.4$\pm$0.3 & 52.3$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 76.9$\pm$0.3 & 61.7$\pm$0.3 \\

==> results/S2/glow_fashionmnist_vs_constant_category_I_bs_5_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 79.9$\pm$0.6 & 64.4$\pm$0.7 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 88.6$\pm$0.4 & 74.7$\pm$0.6 \\

==> results/S2/glow_fashionmnist_vs_mnist_EER_bs_5_10_S2.tex <==
& \textbf{0.9$\pm$0.2} & 5.6$\pm$0.3 & \textbf{0.0$\pm$0.0} & 1.2$\pm$0.2 \\

==> results/S2/glow_fashionmnist_vs_mnist_bs_2_10_S2.tex <==
& \textbf{91.8$\pm$0.1} & \textbf{92.0$\pm$0.1} & 88.9$\pm$0.1 & 81.4$\pm$0.3 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 99.7$\pm$0.1 & 99.6$\pm$0.1 \\

==> results/S2/glow_fashionmnist_vs_mnist_divergence_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 14.7$\pm$0.5 & \textbf{0.0$\pm$0.0} & 7.3$\pm$0.2 \\

==> results/S2/glow_fashionmnist_vs_mnist_divergence_bs_2_10_S2.tex <==
& \textbf{97.1$\pm$0.1} & \textbf{97.3$\pm$0.1} & 73.8$\pm$0.2 & 65.0$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 95.8$\pm$0.5 & 93.6$\pm$1.3 \\

==> results/S2/glow_fashionmnist_vs_notmnist_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 29.5$\pm$0.3 & \textbf{0.0$\pm$0.0} & 20.8$\pm$0.3 \\

==> results/S2/glow_fashionmnist_vs_notmnist_bs_2_10_S2.tex <==
& \textbf{99.3$\pm$0.0} & \textbf{99.4$\pm$0.0} & 63.6$\pm$0.2 & 61.4$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 87.3$\pm$0.3 & 85.6$\pm$0.6 \\

==> results/S2/glow_fashionmnist_vs_notmnist_gray_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 44.5$\pm$0.4 & \textbf{0.0$\pm$0.0} & 39.4$\pm$0.5 

==> results/S2/glow_fashionmnist_vs_notmnist_gray_bs_2_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 23.4$\pm$0.5 & 35.3$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 23.9$\pm$0.6 & 35.5$\pm$0.2 \\

==> results/S2/glow_mnist_only_9_vs_mnist_except_9_bs_5_10_S2.tex <==
& \textbf{95.0$\pm$0.7} & \textbf{95.6$\pm$0.8} & 76.3$\pm$1.5 & 80.2$\pm$1.8 & \textbf{99.7$\pm$0.2} & \textbf{99.7$\pm$0.2} & 80.1$\pm$2.6 &  84.2$\pm$1.9

==> results/S2/glow_svhn_vs_celeba32_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_celeba32_bs_2_10_S2.tex <==
& 99.9$\pm$0.0 & 99.9$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_celeba32_gray_EER_bs_5_10_S2.tex <==
& \textbf{8.0$\pm$0.3} & 43.2$\pm$0.3 & \textbf{2.3$\pm$0.2} & 40.2$\pm$0.8 \\

==> results/S2/glow_svhn_vs_celeba32_gray_bs_2_10_S2.tex <==
& \textbf{96.2$\pm$0.1} & \textbf{96.4$\pm$0.1} & 44.1$\pm$0.3 & 43.8$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 55.0$\pm$0.3 & 49.1$\pm$0.3 \\

==> results/S2/glow_svhn_vs_cifar100_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_cifar100_bs_2_10_S2.tex <==
& 98.9$\pm$0.0 & 99.1$\pm$0.0 & \textbf{99.9$\pm$0.0} & \textbf{99.9$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_cifar100_gray_EER_bs_5_10_S2.tex <==
& \textbf{23.3$\pm$0.4} & 61.0$\pm$0.3 & \textbf{19.4$\pm$0.5} & 68.2$\pm$0.2 \\

==> results/S2/glow_svhn_vs_cifar100_gray_bs_2_10_S2.tex <==
& \textbf{92.3$\pm$0.1} & \textbf{93.2$\pm$0.1} & 41.2$\pm$0.4 & 42.4$\pm$0.2 & \textbf{98.9$\pm$0.2} & \textbf{99.0$\pm$0.2} & 28.0$\pm$0.8 & 36.6$\pm$0.3 \\

==> results/S2/glow_svhn_vs_cifar10_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_cifar10_bs_2_10_S2.tex <==
& 98.9$\pm$0.1 & 99.1$\pm$0.1 & \textbf{99.9$\pm$0.0} & \textbf{99.9$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_cifar10_gray_EER_bs_5_10_S2.tex <==
& \textbf{24.0$\pm$0.5} & 64.1$\pm$0.3 & \textbf{18.7$\pm$0.5} & 70.9$\pm$0.3 \\

==> results/S2/glow_svhn_vs_cifar10_gray_bs_2_10_S2.tex <==
& \textbf{91.8$\pm$0.2} & \textbf{92.7$\pm$0.1} & 37.8$\pm$0.3 & 40.5$\pm$0.1 & \textbf{99.4$\pm$0.0} & \textbf{99.5$\pm$0.0} & 24.8$\pm$0.7 & 35.6$\pm$0.2 \\

==> results/S2/glow_svhn_vs_constant_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_constant_category_I_bs_2_4_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 100.0$\pm$0.0 & 99.9$\pm$0.1 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_constant_category_I_bs_5_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_imagenet32_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_imagenet32_bs_2_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_imagenet32_gray_EER_bs_5_10_S2.tex <==
& \textbf{9.3$\pm$0.2} & 53.7$\pm$0.6 & \textbf{4.0$\pm$0.3} & 56.4$\pm$0.6 

==> results/S2/glow_svhn_vs_imagenet32_gray_bs_2_4_S2.tex <==
& \textbf{90.4$\pm$0.3} & \textbf{89.8$\pm$0.2} & 45.0$\pm$0.4 & 44.6$\pm$0.3 & \textbf{95.6$\pm$0.1} & \textbf{95.0$\pm$0.2} & 43.6$\pm$0.2 & 43.6$\pm$0.1 \\

==> results/S2/glow_svhn_vs_mnist_bs_2_4_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 85.8$\pm$0.2 & 84.8$\pm$0.1 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 94.3$\pm$0.2 & 94.0$\pm$0.3 \\

==> results/S2/glow_svhn_vs_mnist_bs_5_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 96.1$\pm$0.1 & 95.9$\pm$0.2 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 99.4$\pm$0.1 & 99.3$\pm$0.1 \\

==> results/S2/glow_svhn_vs_notmnist_bs_2_4_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 97.9$\pm$0.1 & 98.6$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 99.8$\pm$0.1 & 99.8$\pm$0.0 \\

==> results/S2/glow_svhn_vs_notmnist_bs_5_10_S2.tex <==
& \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 99.9$\pm$0.0 & 99.9$\pm$0.0 & \textbf{100.0$\pm$0.0} & \textbf{100.0$\pm$0.0} & 100.0$\pm$0.0 & 100.0$\pm$0.0 \\

==> results/S2/glow_svhn_vs_uniform_noise_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} & \textbf{0.0$\pm$0.0} \\

==> results/S2/glow_svhn_vs_uniform_noise_gray_EER_bs_5_10_S2.tex <==
& \textbf{0.0$\pm$0.0} & 79.1$\pm$0.6 & \textbf{0.0$\pm$0.0} & 81.7$\pm$0.4 \\
